Automatic Classification of Functional Gait Disorders

This article proposes a comprehensive investigation of the automatic classification of functional gait disorders based solely on ground reaction force (GRF) measurements. The aim of the study is twofold: (1) to investigate the suitability of stateof-the-art GRF parameterization techniques (representations) for the discrimination of functional gait disorders; and (2) to provide a first performance baseline for the automated classification of functional gait disorders for a large-scale dataset. The utilized database comprises GRF measurements from 279 patients with gait disorders (GDs) and data from 161 healthy controls (N). Patients were manually classified into four classes with different functional impairments associated with the "hip", "knee", "ankle", and "calcaneus". Different parameterizations are investigated: GRF parameters, global principal component analysis (PCA)-based representations and a combined representation applying PCA on GRF parameters. The discriminative power of each parameterization for different classes is investigated by linear discriminant analysis (LDA). Based on this analysis, two classification experiments are pursued: (1) distinction between healthy and impaired gait (N vs. GD) and (2) multi-class classification between healthy gait and all four GD classes. Experiments show promising results and reveal among others that several factors, such as imbalanced class cardinalities and varying numbers of measurement sessions per patient have a strong impact on the classification accuracy and therefore need to be taken into account. The results represent a promising first step towards the automated classification of gait disorders and a first performance baseline for future developments in this direction.

==> Automatic Classification of Functional Gait Disorders/01_intro.tex <==
\IEEEPARstart{G}{ait} analysis is a tool for clinicians to objectively quantify human locomotion and to describe and analyze a patient`s gait performance. The primary aim is to identify impairments that affect a patient's gait pattern~\cite{baker_measuring_2013}. 

Recordings obtained during clinical gait analyses produce a vast amount of data which are difficult to comprehend and analyze due to their high-dimensionality, temporal dependences, strong variability, non-linear relationships and correlations within the data\cite{chau_review_2001-1}. This makes data interpretation challenging and requires an experienced clinician to draw valid conclusions. Several automatic analysis approaches based on machine learning have been published in recent years to tackle these problems and to support clinicians in identifying and categorizing specific gait patterns into clinically relevant categories~\cite{chau_review_2001-1},~\cite{chau_review_2001-2}. Machine learning methods employed in this context comprise neural networks~\cite{lozano2010human,zeng2016parkinson,vieira2015software}, support vector machines (SVMs)~\cite{wu2007feature,wu2008pca,levinger2009application}, nearest neighbor classifiers~\cite{mezghani2008automatic,alaqtash2011automatic}, and different clustering approaches (hierarchical, k-means, etc.)~\cite{ferrarin2012gait}. The performance of such methods strongly depends on the input data representation \cite{bengio2013representation}.  Frequently used representations in gait analysis comprise discrete kinematic gait parameters (e.g. local minima and maxima of gait signals and time-distance parameters) \cite{giakas1997time,lafuente_design_1998,alaqtash2011automatic}. Additionally, previous research has shown that global signal representations obtained by principal component analysis (PCA)~\cite{soares2016principal,muniz2009application}, kernel-based~PCA~(KPCA) ~\cite{peng_human_2013,xu_fast_2006} and discrete wavelet transformation~(DWT)~\cite{mezghani2008automatic,alaqtash2011automatic} %and discrete fourier transformation (DFT) 
are suitable for subsequent classification~\cite{soares2016principal,mezghani2008automatic}.

%Three dimensional gait analysis (3DGA) uses motion capturing techniques and the measurement of ground reaction forces (GRF) via force plates to estimate joint kinematics and kinetics. By applying inverse dynamic calculations to the kinematic and GRF data, kinetic quantities such as joint moments and powers can be estimated. Up to date, these measures build the gold standard in clinical gait analysis and allow for the assessment of a large amount of biomechanical gait parameters.The potential drawback of this approach is, that it is a very time consuming, requires highly trained staff to acquire valid and reliable results, and the acquisition costs for the measurement systems are very expensive. In addition 3DGA tools require a complex setup (e.g. calibration, attachment of markers to bony landmarks, etc.). The total of these drawbacks makes such analysis tools often not usable in clinical practice.
%
%The GRF represents the most commonly used biomechanical signals to analyze human gait, because the necessary equipment is affordable and the process of data collection is simple, therefore allowing for high patient throughput.
%
%In routine clinical gait analysis, where clinics have the prerequisite of a high daily patient throughput, typically rather simple assessments are carried out. These involve the quantification  of the ground reaction force (GRF) by force platforms. Changes in the morphology of the GRF waveforms are then related to pathological gait (INLCUDE REF) and information derived from this process is used to inform clinical interventions. 

Typical use cases for automatic gait analysis described in the literature show a moderate to high accuracy in distinguishing between different pathologies or patient groups~\cite{alaqtash2011automatic,muniz2009application,wu2007feature,levinger2009application,wu2008pca,soares2016principal,lozano2010human}. However, most of the existing literature investigated rather simple cases such as the differentiation between the affected/non-affected limb in hemiplegic patients~\cite{lemoyne2014implementation}, and the distinction of healthy gait from people with neurological disorders~\cite{alaqtash2011automatic,zeng2016parkinson}, transfemoral amputation~\cite{soares2016principal}, and lower limb fractures~\cite{muniz2009application,lozano2010human}. 
A more complex study is presented in~\cite{williams2015classification}, where several disorders associated with traumatic brain injuries are classified.
The majority of published articles employed kinematic and kinetic data derived from three-dimensional gait analysis (3DGA), which provide a vast amount of kinematic and kinetic information for multiple joints. Drawbacks of such 3DGA measurement systems are the relatively time-consuming data recording, the need for highly trained staff as well as high acquisition and maintenance costs. Therefore, % As a result,
such analysis tools are often not suitable for daily use in clinical practice.  %\todo[inline]{@brian: calibration as additional problem? Glaube dass ist nicht so relevant}

%\new{To manage the high patient throughput in rehabilitation centers, a probably more practical relevant approach is to combine simple visual inspection or 2D video recordings with the quantification of ground reaction forces (GRF) by force platforms. One drawback of such an approach definitely is loss of clinical relevant and quantifiable information (e.g. gait kinematics), which may increase classification accuracy\cite{schollhorn_identification_2002}. However, such simple approaches are common in clinical practice and on the other hand reduce the above mentioned limitations. Anyway,} 
To manage the high patient throughput in rehabilitation centers, a frequently used approach is to combine simple visual inspection or 2D video recordings with the quantification of ground reaction forces (GRF) by force platforms, as changes in the morphology of the GRF waveforms reflect pathological gait~\cite{muniz2009application,alaqtash2011automatic}. %and can be used to inform clinical decisions.} 
One major drawback of this approach is the loss of clinically relevant and quantifiable information (e.g. gait kinematics), causing a potential decrease in classification accuracy\cite{schollhorn_identification_2002}. However, such simple approaches are common in clinical practice as they overcome the before-mentioned limitations of 3DGA. 
To date, few attempts have been published that use only  
GRF data for automated gait pattern classification \cite{goh_multilayer_2014,soares2016principal}.
%richter_classification_2014 not relevant because vertical jump not gait
%\todo[inline]{neuere Referenzen. Matthias: habe einige refs eingefügt (auch ein paar neue dabei (schon in zotero)} 
Most of these gait classification approaches show promising results. However, the majority of previous works employed relatively small datasets. Alaqtash et al.~\cite{alaqtash2011automatic}, for example, compared the data of 12 healthy adults to those of patients with cerebral palsy and multiple sclerosis (4 patients each), Muniz and Nadal~\cite{muniz2009application} used data from 38 healthy controls and 13 patients with lower limb fracture, and Soares et al.~\cite{soares2016principal} classified GRF data of 20 able-bodied and 12 patients with transfemoral amputation. Such small datasets make it difficult to train robust and reliable classifiers that are applicable in complex real-world scenarios. Furthermore, a majority of studies \cite{muniz2009application,mezghani2008automatic,goh_multilayer_2014} %%richter_classification_2014 not relevant because vertical jump not gait
relies solely on the vertical ground reaction force for classification purposes, rather than considering all available GRF components, including the center of pressure (COP), for a more conclusive picture of the underlying gait pattern. Previous classification attempts mainly focused on the differentiation between specific diseases %, e.g. ~\cite{moustakidis_fuzzy_2010}, 
rather than drawing a distinction between functional gait disorders. 
The work of K\"ohle and Merkl~\cite{kohle2000analyzing, kohle1996identification}, who clustered and classified GRF measurements into deficits of different body regions, represents an exception in this regard.
%\new{Their dataset was about half of the size of the one presented in the present paper and containing also gait data from prosthesis wearer.}
Their dataset was about half of the size of the one presented in this article and their work also focused on patients walking with a prosthesis.
%\todo[inline]{können wir uns noch besser und expliziter abgrenzen von Köhle und Merkl? welche signale? --> 3 GRF komponenten und Torque, wie tiefgehend, bei der Klassifikation? Wie groß der Datensatz? --> um die hälfe kleiner, Wie hoch die deviation from RB?} 
In this article we define a functional gait disorder as the cause of a gait impairment, which is reflected by the individual gait patterns. These may be associated with a patient's condition after joint replacement surgery, fractures, ligament ruptures, osteoarthritis or related disorders. The classification of functional gait disorders is of particular interest in clinical examinations, as it may play a key role in detecting arthropathies or diseases at an early stage. In addition, such a classification may also indicate secondary disorders that otherwise might be easily overlooked during clinical examination.
%a patient may show a primary disorder impairing one's gait, which is accompanied by one or more secondary disorders as well. These however, may be easily overlooked during clinical examination.

%For the purpose of data reduction within these approaches techniques such as principal component analysis (PCA, ~\cite{soares2016principal,muniz2009application}), fast-fourier transformation (FFT, Add Ref) and dynamic wrapping techniques? (DWT - eher dicrete wavelet transform, Add Ref) fast-fourier transformation (FFT, Add Ref)are commonly used.   
%\todo[inline]{Brian: ist die Info über Data recution notwendig? Was meint ihr?} 
%\todo[inline]{@ Brian: Wuerde es wie oben angefuehrt einfuegen = Argument, warum wir diese Verfahren einsetzen...}
%and principal component analysis~\cite{soares2016principal,muniz2009application} among various other methods. In order to extract relevant features 

The aim of this article is to present a detailed investigation of the automated classification of several functional gait disorders solely based on GRF data. %It therefore builds upon early researcher dealing with more simple classification tasks based solely on GRFs.
The presented approach builds upon the aforementioned studies, e.g. \cite{goh_multilayer_2014, muniz2009application, soares2016principal}, investigates the suitability of frequently used state-of-the-art GRF parameterization techniques for gait classification and analyzes their discriminative power. In the experiments we evaluate the individual representations on a large-scale and real-world dataset for different classification tasks. %As a result, t
This paper therefore presents a first performance baseline for the automatic classification of different gait disorders in a real-world setting. %In addition, results obtained in this study may serve as a guide for the future development of useful and simple supportive tools for clinical decision making, solely based on GRF data.

%For our investigation we employ a large-scale and real-world data set of 543 patients provided by the Austrian Workers' Compensation Board (AUVA) which comprises highly accurate GRF recordings of hundreds of patients with different orthopedic impairments. Together with the data we obtain expert annotations of functional gait disorders associated with the hip, knee, ankle joint and calcaneus. Beyond this, a data set of normal gait is provided. This paper presents a first baseline for the automatic classification of general gait disorders and represents a baseline for future research as well as a first step towards a useful support tool for clinicians.

%The main goal of the project is to extend previously established classification approaches by developing robust methods which are able to detect functional gait disorders associated with the hip, knee, ankle joint or calcaneus. This automated classification should then result in a support tool for clinicians. 
%This approach may allow to support clinicians in identifying certain gait-related impairments at the level of the hip, knee, and ankle joints. %This approach may allow to diagnose gait disorders, support clinicians to relate them to a certain impairment rendering possible early interventions. 

%\todo[inline]{Caterine: ... due to injuries in the hip, knee, ankle and calcaneus areas. ??? Oder so. andere klassifizieren wir ja nicht}

%The Workers' Compensation Board1 (AUVA - Allgemeine Unfallversicherungsanstalt) is the social insurance for occupational risks for more than 3.3 million employees and 1.4 million pupils and students in Austria and runs several rehabilitation centers. Their rehabilitation centers (e.g. AUVA, Weisser Hof, in Lower Austria) typically use a combination of the aforementioned force plates to determine GRFs during locomotion and OGA as well as more cost-efficient two-dimensional gait analysis tools to assess the patients gait disorders and to evaluate the patients’ progress during physical therapy treatment.

%In this project the partner AUVA maintains a large dataset of GRF data that contains measurements of patients with different ages, weights, and a broad range of functional deficits as well as detailed clinical diagnoses for each patient. This exceptional dataset bears for the first time the potential to develop novel powerful analysis techniques for gait patterns that fulfill the strong requirements of therapists and clinicians and are thus applicable in clinical daily routine.


%As outlined by Chau~\cite{chau_review_2001-1},~\cite{chau_review_2001} analysis of gait data is a challenging task due to the high-dimensionality, temporal dependences, high variability, nonlinear relationships and correlations within the data. 

%While some articles follow a more extensive approach by using kinematic and kinetic data derived from three-dimensional gait analysis, which provide multivariate…, others are solely based on the measurement of vertical ground reaction forces




==> Automatic Classification of Functional Gait Disorders/04_methods.tex <==
%\IEEEPARstart{M}{ethodology} goes here...

\subsection{Patients and dataset}

%(Describe our data set, where it comes from, what it contains, what types of deficits are there, what kind of annotations do we have, who annotated this...)

The presented retrospective study was approved by the local Ethics Committee of Lower Austria (GS1-EK-4/299-2014). 
The anonymized data used in this study are part of an existing clinical gait database maintained by a rehabilitation center of the Austrian Workers' Compensation Board (AUVA). The AUVA is the social insurance for occupational risks for more than 3.3 million employees and 1.4 million pupils and students in Austria.
% This large data set contains GRF measurements of patients with different ages, body mass, and a broad range of functional gait disorders with detailed clinical diagnoses for each patient (Table \ref{tab:dataset}).
The utilized database comprises GRF measurements from 279 patients with gait disorders (GD) and data from 161 healthy controls (N), both of various physical composition and gender (see Table \ref{tab:data set} for details on the dataset). Patients were manually classified into four classes - calcaneus ``C" (n~=~82), ankle ``A" (n~=~62), knee ``K" (n~=~69), and hip ``H" (n~=~66) - by a physical therapist, based on the available medical diagnosis of each patient. Thus, GD refers to C~$\cup$~A~$\cup$~K~$\cup$~H. The individual GD classes include patients after joint replacement surgery, fractures, ligament ruptures, and related disorders associated with the above-mentioned anatomical areas. The most common injuries present in the hip class are fractures of the pelvis and thigh as well as luxation of the hip joint, coxarthrosis, and total hip replacement. The knee class comprises patients after patella, femur or tibia fractures, ruptures of the cruciate or collateral ligaments or the meniscus and total knee replacements. The ankle class includes patients after fractures of the calcaneus, malleoli, talus, tibia or lower leg, and ruptures of ligaments or the achilles tendon. The calcaneus class comprises patients after calcaneus fractures or ankle fusion surgery. All of the above-mentioned injuries may occur individually or in combination within each class.

%The provided data set contains GRF measurements \textbf{543} of patients of different age, sex, and body mass, with injuries or functional disorders at the hip, knee, ankle joints and at the calcaneus.Apart from these data, the data set contains \textbf{543} measurements for a set of healthy individuals (referred to as NORM).Only data from patients who were able to walk unassisted and without a walking aid over a 10 m walkway were included to remove possible biases in the data set.Patients were manually assigned to one of the four classes (referred  to as HIP, KNEE, ANKLE, CALC) by a physical therapist with more than one decade of experience in gait analysis.
% NEU: These data were used in order to create three initial data sets: A large data set hereafter referred to as data set “A”, a small unbalanced data set hereafter referred to as data set “B” and three small balanced data set hereafter referred to as data set “C1”, “C2” and “C3”.
% NEU: Data set A contains data of all classes (normal and pathological) comprising variable measurement sessions per patient and eight trials per session for the affected and non-affected leg. To receive a large number of measurement sessions of each class the class cardinality was kept unbalanced. 
% NEU: Data set B is a subset of data set A. Only initial measurements were included in this data set hence containing only one measurement session per patient. The class cardinality was kept unbalanced to achieve the maximal amount of data. 
% NEU: The tree data sets C1, C2 and C3 were randomly generated from data set B with the only difference that all classes (normal and pathological) are of the same cardinality. The cardinality was adapted to the smallest data set (27 subjects) thus this data set is completely present in all three data sets C.

%\todo[inline]{@Caterine: wie besprochen Diagnosen in einem Ansatz kurz beschrieben ....}

%Each of these classes contains gait measurements of patients with different functional gait disorders. Detailed clinical diagnoses are provided for each patient. The most common injuries in the area of the hip are different kinds of fractures of the pelvis (pubic bone, hip socket, sacrum, ilium) and thigh (femur, femoral neck) as well as luxation of the hip joint, coxarthrosis and total hip endoprosthesis. The most frequent injuries around the knee comprise fractures or ruptures of the kneecap (patella), fractures of the thigh (femur) or shin (tibia), ruptures of the cruciate or collateral ligaments or the meniscus and total knee endoprostheses.Commonly occurring injuries around the ankle joints are fractures of the calcaneus, malleoli, talus, tibia or lower leg and ruptures of the ligaments and the Achilles tendon. In the class of the calcaneus injuries (CALC) fractures and stiffening of the calcaneus (arthrodesis) occur most often. All of the mentioned injuries may occur individually or in combination within each class.  

%The dataset contains a total of N different diagnoses which were assigned to the four classes HIP, KNEE, ANKLE, CALC.

%\todo[inline]{Anmerkung Matthias: hier wuerde ich auf jeden Fall den groesten Datensatz beschreiben (A). Auf die anderen werden wir dann bei Bedarf verweisen.}

Each patient performed one or several measurement sessions. In each session, eight recordings for two consecutive steps were performed. Each bilateral recording is referred to as one trial in this paper. Thus, the utilized dataset contains 1,187 sessions comprising 9,496 individual trials (see Table \ref{tab:data set} for details).
% , which were assigned to five classes: a normative data set (NORM) and four different gait disorder classes. These contain data of patients with impairments \todo{injuries ??? die impairments sind die Folgeerscheinung der Verletzungen, oder?} associated with the calcaneus (CALC) or the ankle (ANKLE), knee (KNEE) and hip (HIP) joints. Patients were manually classified to one of the four classes by a physical therapist with more than one decade of experience in gait analysis. In detail ... 
\begin{table*}[ht!]
\centering
\caption{Details of the dataset and classes}
\label{tab:data set}
\begin{tabular}{lcccccc}
\hline
Class & Amount & \begin{tabular}[c]{@{}c@{}}Age (yrs.)\\ Mean $\pm$ SD\end{tabular} & \begin{tabular}[c]{@{}c@{}}Body Mass (kg)\\ Mean $\pm$ SD\end{tabular} & \begin{tabular}[c]{@{}c@{}}Sex\\ (m/f)\end{tabular} & Num. Sessions & Num. Trials \\
\hline
\rowcolor{gray!15}
Healthy Control (N) & 161 & 32.4 $\pm$ 13.6 & 74.1 $\pm$ 16.2 & 84/77 & 161 & 1,288 \\
Calcaneus (C) & 82 & 42.4 $\pm$ 9.9 & 84.5 $\pm$ 12.1 & 74/8 & 320 & 2,560 \\
\rowcolor{gray!15}
Ankle (A) & 62 & 40.0 $\pm$ 11.5 & 88.3 $\pm$ 16.9 & 56/6 & 259 & 2,072 \\
Knee (K)& 69 & 41.5 $\pm$ 11.4 & 83.7 $\pm$ 19.6 & 44/25 & 258 & 2,064 \\
\rowcolor{gray!15}
Hip (H) & 66 & 43.6 $\pm$ 14.7 & 81.6 $\pm$ 18.3 & 53/13 & 189 & 1,512 \\ \hline
\textbf{SUM} & \textbf{440} & \textbf{38.4} \textbf{$\pm$ 13.3} & \textbf{80.7} \textbf{$\pm$ 17.3} & \textbf{311/129} & \textbf{1,187} & \textbf{9,496} \\ \hline
\end{tabular}
\end{table*}

%Apart from standard data of healthy individuals there are four data sets of persons with injuries or functional disability in the area of the hips, knees, ankles or heel bones. While/whereas healthy persons mostly show natural and symmetrical gait pattern persons with injuries or functional disability often display deviations from normal gait patterns related to physical constraints/limitations. 

%\todo[inline]{will we use different datasets or not?} %Matthias: I propose to use Dataset A and to provide remarks to Dataset B and C where necessary. But the main focus is the large dataset. Datasets B and C are just necessary to show that repeated measurements and class balance have been considered.
%\todo[inline]{todo later: there a 3 dataset: a b and c. a=all data: repeated measurement sessions, imbalanced classes, b=1measurement session per person, imbalanced, c=1session, balanced. why 3 datasts? to enable a more comprehensive statistical analysis and to investigate investigate the effect of class balance and repeated measurements.}
%The data of all classes (normal and pathological) include one or several measurement sessions per patient and ten trials per session. Parts of the data of the four pathologic classes include annotations regarding the affected leg/side. Additional the four pathologic classes may contain annotated data of sessions performed with walking aids like walker-rollator, crutch or cane. Walking aids serve as support for partial or full body weight relief and for balance. The class cardinality is unbalanced.These data were used in order to create three initial data sets: A large data set hereafter referred to as “data set A”, a small unbalanced data set hereafter referred to as “data set B” and a small balanced data set hereafter referred to as “data set C”.

%\subsubsection{Large dataset – data set A (CS)}
%variable number of measurement sessions per patient, unbalanced class cardinality)\\
%Data set A is a subset of the total data described in the previous paragraph. It contains data of all classes (normal and pathological) comprising variable measurement sessions per patient and eight trials per session. From the four pathologic classes only measurements with annotations concerning the affected legs were included and of these only the data of the affected side. As full body weight is essential for gait data analysis measurements carried out with the help of walking aids were - due to the relief of the bodyweight – excluded in this data set. To receive a large number of measurement sessions of each class the class cardinality was kept unbalanced. 

%\subsubsection{Small unbalanced dataset – data set B (CS)}
%(1 measurement session per patient, unbalanced class cardinality)\\
%Data set B is a subset of data set A. Only initial measurements were included in this data set hence containing only one measurement session per patient. The class cardinality was kept unbalanced to achieve the maximal amount of data. 

%\subsubsection{Small balanced dataset – data set C (CS)}
%(1 measurement session per patient, balanced class cardinality)\\
%Data set C is a subset of data set B. It is equal to data set B with the only difference that all classes (normal and pathological) are of the same cardinality.\\


%Which datasets do we use for what investigation (and why)?
\subsection{Data recording and preprocessing}
Gait analysis was performed on a 10m walkway with two centrally embedded force plates (Kistler, Type 9281B12). 
%\new{The force plates were placed in a consecutive order and flush with the ground, so that a person can walk across both force plates by placing one foot on each plate. Both plates were covered with the same walkway surface material, so that targeting was not an issue.} 
The force plates were placed in a consecutive order, allowing a person to walk across by placing one foot on each plate. Both plates were flush with the ground and covered with the same walkway surface material, so that targeting was not an issue.
During a session, participants walked unassisted and without a walking aid at a self-selected walking speed until a minimum of eight valid recordings were available. 
These recordings were defined as valid by a supervisor when the participant walked naturally and there was a clean foot strike on the force plate.
Prior to the gait analysis session, each participant underwent rigorous physical examination by a physician. 

All processing steps and subsequent analyses were performed in Matlab 2016a (The MathWorks Inc., Natick, MA, USA). The three analog GRF signals as well as the two COP signals were converted to digital signals using a sampling rate of 2000Hz and a 12-bit analog-digital converter (DT3010, Data Translation Incorporation, Marlboro, MA, USA) with a signal input range of $\pm$10V. A threshold of 10N was used for step detection and 30N for COP calculation. Raw signals were filtered using a 2nd order low-pass butterworth filter with a cut-off frequency of 20Hz. All gait measurements were temporally aligned so that they all started with the initial contact and ended with toe-off. They were further time-normalized to 100\% stance by re-sampling the data to 1000 points. The processed signals are referred to as waveforms in this article. Amplitude values of the three force components, i.e. vertical (V), medio-lateral (ML), and anterior-posterior (AP), were expressed as a multiple of body weight ($BW$) by dividing the force by the product of body mass times acceleration due to gravity ($g$). The COP waveforms from each trial were normalized by the foot length ($FL$) determined during each session, expressed as a multiple of foot length.


\subsection{Signal representation}
The representations employed in our investigation comprise (1)~discrete GRF parameters ~(DP) in combination with time-distance parameters~(TDP) \cite{lafuente_design_1998, alaqtash2011automatic,giakas1997time}; (2)~PCA-based parameterizations of the entire GRF waveforms \cite{lozano2010human,soares2016principal,wu2008pca} and (3)~a combination of the first two approaches, i.e. PCA applied to %on 
DPs and TDPs \cite{wu2007feature}. In the following, all three approaches are described in detail.

DPs were calculated for the affected limb and extracted from all three force components, $F_{V}(t)$ (vertical), $F_{AP}(t)$ (anterior-posterior), and $F_{ML}(t)$ (medio-lateral), as well as from the COP displacement in the anterior-posterior (walking) direction $COP_{AP}(t)$ and in the medio-lateral direction $COP_{ML}(t)$. An example of the GRF and corresponding COP waveforms is presented in Figure \ref{img:GRFcomp}. Furthermore, a more detailed visualization of the mean GRF waveforms over each class is illustrated in Figure S1 (supplementary material). DPs include a set of predefined (most prominent) local minima and maxima of the waveforms, which were extracted by peak detection in a fully automatic way from each trial. Furthermore, impulses were calculated over different segments of the waveform by multiplying the average force (in $N$) by the time this force is active. To account for differences in body mass between participants \cite{moisio_normalization_2003}, all impulses were  divided by the product of body mass times acceleration due to gravity~($g$) and then multiplied by 100 ($\%BW\cdot$$s$). TDPs such as cadence~($CAD$), double support time~($DS$), gait velocity~($GV$), step length~($STEPLEN$), and stance time~($ST$) were calculated from two consecutive steps (affected and unaffected limb) and averaged over the eight valid trials. Table \ref{tab:GRFparams} lists all 52 extracted parameters.

\begin{figure}
  \centering
	\includegraphics[width=0.90\linewidth]{images/GRFSignals}
    \caption{(top) The characteristic shape of the three components of the GRF: the vertical force ($F_{V}$), the anterior-posterior shear ($F_{AP}$), and the medio-lateral shear ($F_{ML}$). (bottom) The corresponding COP path for one step. Note that x and y axes are scaled slightly differently for better visualization.}
    \label{img:GRFcomp}
\end{figure}

\begin{table*}[ht!]
\centering
\caption{Discrete and time-distance parameters, description, type of normalization and physical unit.}
\label{tab:GRFparams}
\resizebox{.80\textwidth}{!}{%
\begin{tabular}{llll} %{p{1.6cm}p{18.0cm}p{2.0cm}p{1.0cm}}
\hline
Abbreviation		&	Description                                            								&	Normalization 		& 	Unit 	\\ \hline
\rowcolor{gray!15}
$ST$				&	Stance time is the duration of the stance phase	of one foot										&	-					&	$s$\\
$F_{V1}$		& 	Maximum value of $F_{V}$ within the breaking phase of stance													&	Body weight			&	$BW$\\
\rowcolor{gray!15}
$T_{V1}$     	&  	Time of $F_{V1}$																				&	Stance time			&	\%ST\\
$F_{V2}$   		&   Minimum value of $F_{V}$ between $T_{V1}$ and $T_{V3}$											&	Body weight			&	$BW$\\
\rowcolor{gray!15}
$T_{V2}$    	&   Time of $F_{V2}$																				&	Stance time			&	\%ST\\
$F_{V3}$  		&	Maximum value of $F_{V}$) within the propulsive phase of stance													&	Body weight			&	$BW$\\
\rowcolor{gray!15}
$T_{V3}$ 		&	Time of $F_{V3}$																				&	Stance time			&	\%ST\\
$F_{AP1}$		&	Maximum value of $F_{AP}$ between initial contact and $T_{AP2}$								&	Body weight			&	$BW$\\
\rowcolor{gray!15}
$T_{AP1}$		&	Time of $F_{AP1}$																				&	Stance time			&	\%ST\\ 
$F_{AP2}$		&	Minimum value of $F_{AP}$) within the breaking phase of stance 		 							&	Body weight			&	$BW$\\ 
\rowcolor{gray!15}
$T_{AP2}$		&  	Time of $F_{AP2}$              																	&	Stance time			&   \%ST\\
$F_{AP3}$		&	Maximum value of $F_{AP}$) within the propulsive phase of stance									&	Body weight    		&   $BW$\\
\rowcolor{gray!15}
$T_{AP3}$		&	Time of $F_{AP3}$                     															& 	Stance time			&   \%ST\\
$F_{ML1}$		&	Minimum value of $F_{ML}$ within the breaking phase of stance				           			&	Body weight			&	$BW$\\
\rowcolor{gray!15}
$T_{ML1}$		&	Time of $F_{ML1}$												                      			&   Stance time			&	\%ST\\
$F_{ML2}$		&	Maximum value of $F_{ML}$ within the breaking phase of stance									&	Body weight     	&	$BW$\\
\rowcolor{gray!15}
$T_{ML2}$		&	Time of $F_{ML2}$          												            			&   Stance time			&	\%ST\\
$F_{ML3}$		&	Maximum value of $F_{ML}$ within the propulsive phase of stance									&	Body weight			&	$BW$\\
\rowcolor{gray!15}
$T_{ML3}$		&	Time of $F_{ML3}$        												              			&	Stance time			&	\%ST\\
$F_{VAVG}$ 		&	Mean value of $F_{V}$																			&	Body weight   		&	$BW$\\
\rowcolor{gray!15}
$F_{APAVG}$ 	&	Mean value of $F_{AP}$																			&	Body weight			&	$BW$\\
$F_{MLAVG}$ 	&	Mean value of $F_{ML}$																			&	Body weight			&	$BW$\\
\rowcolor{gray!15}
$IF_{V}$ 		&	Impulse of $F_{V}$ during stance				 										&   Body weight            		&   $\%BW\cdot$$s$\\	
$IF_{AP}$    	&	Impulse of $F_{AP}$ during stance													&   Body weight            		&   $\%BW\cdot$$s$\\
\rowcolor{gray!15}
$IF_{ML}$   	&	Impulse of $F_{ML}$ during stance													&   Body weight            		&   $\%BW\cdot$$s$\\
$IF_{V1}$ 		&	Impulse of $F_{V}$ between initial contact and $T_{V1}$ 	    						&   Body weight            		&   $\%BW\cdot$$s$\\
\rowcolor{gray!15}
$IF_{V2}$ 		&	Impulse of $F_{V}$ between initial contact and $T_{V2}$ 	  							&   Body weight            		&  	$\%BW\cdot$$s$\\	
$IF_{V3}$  		&	Impulse of $F_{V}$ between initial contact and $T_{V3}$ 	  							&   Body weight            		&  	$\%BW\cdot$$s$\\
\rowcolor{gray!15}
$IF_{APDEC}$	&	Impulse of $F_{AP}$ during the breaking phase										&   Body weight            		&  	$\%BW\cdot$$s$\\     
$IF_{APACC}$	&	Impulse of $F_{AP}$ during the propulsive phase 										&   Body weight            		&  	$\%BW\cdot$$s$\\   
\rowcolor{gray!15}
$IF_{LAT}$   	&	Impulse of the lateral component of $F_{ML}$											&   Body weight            		&  	$\%BW\cdot$$s$\\
$IF_{MED}$   	&	Impulse of the medial component of $F_{ML}$    	         							&   Body weight            		&	$\%BW\cdot$$s$\\
\rowcolor{gray!15}
$COPANG$          &	COP angle is the horizontal angle between the COP linear regression line and the x-axes ($\neq$ foot rotation)					&   -            		&   deg \\
$COPDEV$          &	COP deviation is the root mean square error of the COP linear regression 						&   Foot length            		&   $FL$ \\
\rowcolor{gray!15}
$COP_{AP}$         	&	COP range is the range in the anterior-posterior direction during stance phase                    														&   Foot length            		&	$FL$ \\
$COPV$   			&	COP velocity is calculated as the ratio of foot length and stance time 							      											&   Foot length            		& 	$FL/s$\\
\rowcolor{gray!15}
$COP_{ML}$          	&	COP range is the range in the medio-lateral direction during stance phase                 							&   Foot length            		& 	$FL$\\
$DECT$      		&	Deceleration time (breaking phase) is the duration of $F_{AP}$ being negative                   &   -            		&   $s$\\
\rowcolor{gray!15}
$ACCT$       		&	Acceleration time (propulsive phase) is the duration of $F_{AP}$ being positive        			&   -            		&   $s$\\

$LR0080$   		&	Loading rate represented as the slope of $F_{V}$ from the initial contact to 80\% of $F_{V1}$	&   Body weight            		& 	$N/s$\\
\rowcolor{gray!15}
$LR2080$  		&	Loading rate represented as the slope of $F_{V}$ from 20\% to 80\% of $F_{V1}$											&   Body weight            		&   $N/s$\\

$UR8000$     		&	Unloading rate represented as the slope of $F_{V}$ from 80\% of $F_{V3}$ to the toe-off         &   Body weight            		&   $N/s$\\

\rowcolor{gray!15}
$UR8020$     		&	Unloading rate represented as the slope of $F_{V}$ from 80\% to 20\% of $F_{V3}$                 						&   Body weight            		&   $N/s$\\

$DS$     			&	Double support time during one stride														&   -            		&   $s$\\
\rowcolor{gray!15}
$STEPLEN$			&	Step length is the distance of the COP position from initial contact to following contralateral initial contact &   -      				& 	$m$\\

$STEPV$ 			&	Step velocity is calculated as the ratio of step length and step time								&	-					& 	$km/h$\\
\rowcolor{gray!15}
$STRIDET$         	&	Stride time is the duration from initial contact to initial contact of the ipsilateral foot 		&	-					& 	$s$\\
$BF$        		&	Basic frequency is the mean number of strides per second (1/$STRIDET$)                          	&	-					& 	$Hz$\\
\rowcolor{gray!15}
$CAD$          	&	Cadence is the number of steps per minute														&   -            		&	$1/min$\\
$STEPWD$    		& 	Step width is the medio-lateral distance of the mean COP between both feet						&   -           	 		&	$m$	\\
\rowcolor{gray!15}
$STRLEN$  		&	Stride length is the distance of the COP position from initial contact to following ipsilateral initial contact 		&  -             		&	$m$	\\
$GV$				&	Gait velocity is calculated as the mean step velocity of both feet									&	-					&	$km/h$\\ \hline

%\multicolumn{4}{l} {Abbreviations} \\
\multicolumn{4}{l} {Body weight (BW): product of body mass and acceleration due to gravity;} \\
\multicolumn{4}{l} {\%ST: percentage of stance time; \%BW: percentage of body weight; FL: multiple of foot length.}

\end{tabular}% <------ Don't forget this %
}
\end{table*}

In contrast to the GRF parameters (DPs and TDPs), the PCA takes the entire waveforms\footnote{For the purpose of the present study, every third sample was used in order to reduce redundancy in the data, thereby improving the robustness of the decomposition.} of the affected limb into account and %thus 
provides a holistic representation of the data. %Thereby, c
Complementary information to the parameters is thus captured. The main goal of PCA is to reduce the dimensionality of a dataset by transforming the data into a set of uncorrelated variables, i.e. the principal components (PCs) \cite{jolliffe2002principal}. Each PC points in (and thus explains) one orthogonal direction of variance in the data. %PCA explains only linear relationships in the data. To capture higher-order relationships we further employ kernel-PCA with different kernels (polynomial, Gaussian) to obtain better adapting representations. Furthermore, recent literature suggests that KPCA might perform slightly better than PCA as it is not as sensitive to noise~\cite{cao_comparison_2003,xu_fast_2006}. 
%
%Next to several advantageous of the PCA, one major limitations is its sensitivity to noise. One method to bypass this shortcoming is the kernel-based (KPCA, ~\cite{xu_fast_2006}. It utilizes kernel function to gain a random high-order correlation between input variants and finds the PCs need through the inner production between the input data. 
%
The main intention is to obtain a lower-dimensional representation of our time- and weight-normalized waveforms similar to \cite{lozano2010human,soares2016principal,wu2008pca} by projecting the data onto those PCs which explain most variance in the data. This dimensionality reduction fosters subsequent machine learning\cite{chau_review_2001-2}. 
We performed PCA on each of the five signals separately and concatenated the resulting PCs to obtain a feature vector for classification. This approach proved to be superior to other PCA-based representations in a preliminary study~\cite{slijepcevic2017ground}.
The final dimensionality of the obtained representations is specified by the amount of variance preserved in a particular projection, i.e. 98\%, 95\%, and 90\%. An exemplary visualization of the different PCA representations is presented in Figure S2 (supplementary material). 
A preliminary evaluation indicated that preserving 98\% of the variance results in a good trade-off between data reduction and classification performance. Thus, all results presented in the following are based on the approach in which 98\% of the variance is preserved (the number of resulting PCs is waveform-specific and ranges from four to twelve. For all five signals there are 39 PCs in total). 

As a third representation, PCA was applied to the previously extracted DPs and TDPs (a vector comprising of 52 parameters), similarly to Wu et al. \cite{wu2007feature}. This approach combines both methodologies and aims at extracting the most important information from the (possibly redundant) parameters. %By selecting only a subset of the resulting PCs (preserving 98\% of the variance) noise components are removed. This approach implicitly leads to a selection of the most important GRF parameters. 

%Which parameters do we employ? How do we extract them?
%Variants A,B,C: not in this paper
%PCA-Feature computation

\subsection{Statistical analysis}

Our first aim was to investigate the suitability of different parameterization techniques for subsequent gait classification. For this purpose we analyzed the variance and discriminative power of each DP and TDP across the different classes by descriptive statistics in a first step. We calculated the median, interquartile-range (IQR) and range of each parameter within each class and visualized them as boxplots. This enabled us to visually inspect variances and distributions in and across the classes, thereby allowing a first estimation of the discriminative power of each parameter.

In a second step, we investigated the discriminative power of the parameters and the global PCA-based representations by linear discriminant analysis~(LDA). A natural measure to describe the separation of two distributions (classes) is the Fisher criterion, which represents the core of LDA \cite{duda2012pattern}. We applied (multi-class) LDA to assess the discriminative power of individual parameters for two (or more) classes. The advantage of this approach is that the discriminative power of a parameter (even across multiple classes) can be expressed by one scalar value that directly reflects the statistical  properties of the input data. %Hence, no additional modeling or data transformation is applied like in other methods such as SVM, that may additionally influence results. 
Hence, there is no need to apply additional modelling and data transformations (which may influence results) prior to LDA, which would be necessary for other methods such as SVM. Furthermore, this approach can easily be extended to estimate the discriminative power of a combination of several parameters by multi-dimensional LDA (e.g. in case of PCA-based representations). We computed the accuracy of LDA and reported the divergence from a random baseline \cite{Vries2012document} to quantify to which degree an input parameter or input representation is able to separate the underlying classes. The random baseline was estimated by the zero rule (always choosing %guessing 
the most frequent class in the dataset). Thus, in the case of five classes where the largest class contains 30\% of the data the random baseline equals %to 
30\%. 

%For this purpose we analyzed the intra-class \textit{variability} and the inter-class \textit{discriminativity} of the extracted parameters. %We investigate the variability of each parameter across subjects and trials for each class of deficits and estimate the measurement error (in terms of standard error of measurement, SEM). 

%The joint analysis of variability and discriminativity reveals how robust a parameter can be extracted from the data, how sensitive it is to intra-class variations and how different the data distributions vary between the classes of gait disorders and normal gait. 

%To quantify the variability the amount of subject, time and error variation (for each parameter and class) were calculated. This was performed by using the mean square terms (MS\textsubscript{subject}, MS\textsubscript{time}, and MS\textsubscript{error}) of a repeated measures analysis of variances (ANOVA) and dividing them by the respective degrees of freedom in the data. From the resulting variance estimates we took the square root to obtain standard deviations $SD\textsubscript{subject}$, $SD\textsubscript{trial}$, and $SD\textsubscript{error}=SEM$. 
%Since different parameters live in completely different value ranges and physical units, their variability can hardly be compared. One solution is to compute the coefficient of variation (COV). Since our parameters include also negative values, COV is however is not appropriate. To enable an objective comparison between the parameters we divide the standard deviations by the corresponding SEM ($SD\textsubscript{error}$). By this procedure we express variability as a multiple of the measurement error which brings all variabilities into a comparable value range and thereby enables comparisons of subject and trial variability across parameters.
%The discriminativity of parameters across classes is the second important aspect investigated in the statistical analysis. 

%In a first preliminary step, we investigate the variability and discriminativity of different parameters by descriptive statistics. For this purpose we summarize the distributions of the parameters by boxplots which enable us to visually compare variability and discriminativity across the classes.



% LDA served as a classifier (on the whole dataset), rather than computing fisher's criterion, as it was sufficient to determine the discriminativity of a parameter. 

\subsection{Classification}

We applied two classification tasks to the dataset by using SVMs as classifiers: (1) (binary) classification between normal gait and all gait disorders ($N/GD$) and (2) (multi-class) classification between N and each of the four GD classes  ($N/C/A/K/H$). In the first task, the class priors are imbalanced, i.e. there are many more observations in the combined GD class than in the normal class (see Table \ref{tab:data set}). The second task separates each type of disorder from each other and from the normal class. %This is challenging as we expect the classes to mutually overlap in parameter space.

For the classification experiments the dataset was split into a training (65\%) and a test set (35\%), thereby mutually disjoining the groups of patients in both sets. %in such a way that the groups of patients in both sets are mutually disjoint. 
The training dataset in combination with a k-fold cross-validation approach served to train the classifiers and to optimize their parameters (model selection), whereas the test dataset was used to evaluate the generalization ability of the trained models (and was not considered during model selection and hyper-parameter optimization).
The calculated DPs and TDPs as well as the PCA-based representations served as input to classification. The parameters (DPs and TDPs) were normalized (each independently) in a twofold way, by min-max normalization and z-standardization, in order to determine the more suitable approach. The PCA representations were z-standardized. We employed SVMs for the classification with linear and radial basis function (RBF) kernels, provided by the LIBSVM library \cite{ChangLIBSVM2011}. For hyper-parameter selection we applied a grid search over the regularization parameter $C \in [2^{-5}, 2^{15}]$ for the linear SVM and over $C \in [2^{-1}, 2^{15}]$ and the kernel hyper-parameter $\gamma \in [2^{-15}, 2^{5}]$ for the RBF SVM. During the grid search, a 5-fold cross-validation was performed on the training dataset. Finally, an SVM with the best parameters estimated during model selection was trained on the entire training set and evaluated on the test set. Additionally a k-nearest neighbor (k-NN) classifier and a multi-layer perceptron (MLP) were employed as a reference to compare their results to the performance of the SVM. Grid search was performed over various values of k for the k-NN. For the MLPs different numbers and sizes of hidden layers were employed.
As a performance measure we use the classification accuracy, which is the percentage of correct classifications among all classes and input samples. Since in different experiments the random baseline varies, the absolute values of accuracy are of limited expressiveness. To enable a fair comparison, we employ the \emph{divergence from a random baseline} approach  \cite{Vries2012document} and thus provide for each experiment the difference between the random baseline and the absolute classification accuracy. 
%We used the classification accuracy (percentage of correct classifications among all classes) as a performance measure.}







==> Automatic Classification of Functional Gait Disorders/05_results.tex <==
%\IEEEPARstart{I}{n} this section we present the results of our statistical analysis (parameter variability and discriminativity) and first baseline results for the classification of functional gait disorders.  We couple the discussion with each result as they are tightly related.

\IEEEPARstart{T}{his} section presents and discusses the results of the statistical analysis and the classification experiments.

%\todo[inline]{Brian: In unserer Community sind solche allg. Absätze nciht so gerne gesehen?! Djordje: Ich finde es ganz gut, da der Leser moeglicherweise erwartet eine Results- und Disscussion-Subsektion vorzufinden und wir hier erklearen, dass das zusammengeführt wurde.}

% REMOVED: we will publish this separately in a short notice.
% \subsection{Parameter Robustness (DS+All)}

% \begin{itemize}
% \item For which parameters is the difference in the three computation methods A B and C (average curve, averages of parameters, most representative curve) below or above the MDC (Minimal Detectable Change).
% \item If difference below MDC
% \end{itemize}

\subsection{Statistical analysis}

%Figure \ref{img:variability} shows descriptive statistics in terms of boxplots for a subset of the extracted parameters\footnote{Results for all parameters are provided as supplemental material.}. From the boxplots we observe different patterns for the individual parameters..
%\todo[inline]{Info fuer Boxplot-Kategorisierung: \textbf{A:} H+K vs. C+A, \textbf{B:} N vs. HKCA, \textbf{C:} alle gleich, \textbf{D:} H+K aehnlich und C+A unterschiedlich, \textbf{E:} unterschiedliche Variabilitaet; \textbf{F:} A anders und alle anderen gleich, \textbf{G:} N anders und H anders alle anderen gleich} 
%In-depth comprehension/knowledge of the data’s characteristics may be essential in order to identify relevant parameters that further allow for reliable classification results. Thus, a low intraclass variability combined with significant deviations of the mean across classes are expected to reveal best classification results. Analysis of the present data set renders possible the identification of seven subgroups within the pool of variables/ with similarly behaving parameters. An example for each of the identified subgroups as well as characteristic features are discussed below. 
The statistical analysis aimed at assessing the suitability of the individual GRF parameters (DPs and TDPs) for distinguishing different classes of gait disorders. In order to be considered %as 
a "good" parameter, intra-class variation should be low (e.g. small IQR inside a given class), while the inter-class variation should be high (e.g. significantly different means or medians between the samples of different classes) \cite{lafuente_design_1998}.
%
%For this purpose of classification, a parameter which shows a significant deviation of the distribution's central tendency and a minimum overlap of its distribution across different classes is expected to have the most discrimination potential~\cite{lafuente_design_1998}. 
%

The visual inspection of the boxplots for each parameter enables a first assessment of the intra- and inter-class variation and thereby gives an impression of the parameters' potential to differentiate between different classes. Figure~\ref{img:variability} shows boxplots for selected parameters. A presentation of boxplots for all 52 investigated parameters for all classes is provided in Figure S3 (supplementary material). 
%descriptive statistics was conducted to determine parameters behaving similarly. This step allowed for a first estimate of the parameter discrimination potential prior to applying classification procedures. Figure \ref{img:variability} shows boxplots for a subset of the extracted parameters\footnote{Results for all parameters are provided as supplemental material.}: 
Parameters such as $F_{V3}$ (see Figure~\ref{img:variability}(a)) show a clear difference in the median and the IQR between the healthy controls and all four GD classes. This indicates a high potential to discriminate between normal gait and arbitrary gait disorders. 
% Note this can also be seen in the LDA results! The parameter alone yields the best results among all other parameters
However, the overlap of the distributions within the GD classes indicates a low potential to discriminate between them. Other parameters such as $T_{AP3}$ (see Figure~\ref{img:variability}(b)) vary strongly in the IQR and the median across the classes. While the IQR is high for calcaneus and ankle, the classes hip, knee, and the normal controls exhibit a very similar distribution. Thus, such a parameter has solely limited potential to separate normal gait from general gait disorders. There may be, however, a certain potential to separate individual classes (in this case calcaneus) from other classes. 
%show a very high IQR for specific GD sub-categories (calcaneus and ankle) which indicates a low discriminative potential between these categories. 
Other parameters may lack in discriminative power. An example is $IF_{AP}$ (see Figure~\ref{img:variability}(c)), which shows a similar median and overlapping distributions with a similar IQR across all classes.
%Another repeatedly observed parameter behavior refers to the responsiveness toward impairments of a specific area, such as the calcaneus or ankle joint (i.e. $T_{AP3}$). For this parameter, the calcaneus and ankle subgroup show a high IQR, thus indicating a high variability within both groups, while the IQR of all other subgroups stays narrow. In this case, the parameter may have the potential to discriminate the hip, knee, and healthy gait subgroups from the calcaneus and ankle group. 
%The visual inspection via the boxplots allowed to have a more closer look at the data distributions, and can help to identify potential highly discriminating parameters.
Several parameters are discriminative for particular classes or a group of classes. However, none of the observed parameters discriminates well between all classes. Therefore, the combination of several parameters for the distinction between classes seems advisable. %This suggests the combination of several parameters for the distinction between gait classes. 
These assumptions are further corroborated by the LDA results.

\begin{figure}[h!]
  \centering
	\includegraphics[width=0.95\linewidth]{images/boxplots}
    \caption{Example of boxplots for three parameters. Each boxplot shows the median and the IQR (box) for each class (outliers were removed for better visualization). Box-whiskers correspond to 1.5 of the box-length, thus show approximately $\pm$~2.7 standard deviations. The overlap of distributions between the classes gives an impression of the parameters' discriminative power.}
    \label{img:variability}
\end{figure}

%The observation that all four subgroups deviate from normal gait data - as it is the case for parameters TV3, FV3, and UR8020 - may imply that the parameter is suitable for discriminating between normal and disordered gait. With regard to its median, parameter FV3 may potentially allow to make a further distinction between normal gait versus disorders related to either the calcaneus and ankle joint or the hip and knee joint. However, when looking at the interquartile range (IQR) one can observe an overlap between the data of the four subgroups. This overlap may counteract the discriminative power and thus lower the discriminative potential of the according parameter as Lafuente et al. ~\cite{lafuente_design_1998} point out.   

%or solely the ankle joint (parameter COPANG). However, the wide IQR indicates a high variability within these groups and consequently may affect its discriminative power. Even more frequently some subgroups show similar characteristics of parameter behavior, while only one group differs (as observable in parameters LR0080 and STEPWD). Even if this observation may lower overall discriminativity, a deviation of only one group from the other similarly behaving groups may be andvantageous for classification of the specific group (Reference). 

%In contrast, parameter TAP3 seems to be sensitive toward impairments of the calcaneus and ankle joint as opposed to parameter COPANG, which solely seems to be responsive to ankle injuries. 
%As such, figure XX (B) shows an example of the median differing considerably between normal gait data and those of all four subgroups, thus being a prerequisite for classification between normal and disordered gait. 
%Another example is shown in figure XX (A), again showing a clear deviation between normal and disordered gait data. However, on closer inspection the median and IQR of the calcaneus and ankle as well as knee and hip group seems to behave similarly, being an indicator for possible analogies between these subgroups.


%\begin{itemize}
%\item As such, figure X presents an example for pattern/group A, which can be specified by similar parameter behavior in the ankle and calcaneus data and the knee and hip data. However, there is a clear distinction between the mean of the normal versus ankle/calcaneus and knee/hip categories.
%\end{itemize}

% \begin{itemize}
% \item First: explain what we want: low variablity inside class, strong differences in mean across classes.
% \item One approach is to: Identify groups of similarly behaving parameters and discuss these groups.
% \item Which parameters have highest variation, which lowest.
% \item What global patterns are there (e.g. normal class ist most often different, Calc and Ankle are often similar as well as Hip and Knee are often similar. Some parameters have equal distributions across all classes, discuss parameters with completely unique distributions...
% \item Which class produces the strongest variabilities?
% \item Compare variability between NORM class all others. Any patterns and regularities? 
% \item Try to explain why some parameters are better than others? Does it have something todo with the force component, i.e. vertical is better then AP or ML?
% \end{itemize}



%\begin{itemize}
%\item General: If SEM is high for a certain class, then this parameter is suboptimal to judge rehabilitation progress. We want low SEM. How large is the measurement error (i.e. the portion of the measurement error from the total variation)? Which parameters can be estimated most robustly which not? Are there class-specific variations of SEM?  
%\item How large is the variability over patients and trials? Large variability means either: prone to noise or: sensitive to intra-class variations. For classifications we want low intra-class variability. Which parameters have highest variation, which lowest. How robust are the parameters for subject-based variations? For which parameters is the variability over trials higher than over patients? Are there class-specific patterns in variability? Which of the 3 force components produces strongest variability in the parameters?

%\end{itemize}
%\todo[inline]{Cat: generate figure with box plots. I think we need to include PCA here as well! Otherwise the paper gets somehow imbalanced}
%\todo[inline]{Djorde: generate figures for all 3 datasets (100\% variance plot + nCakh-Plot. For dataset C: 3 plots (for each sample set C1, C2, C3 one). Note: for smallest class there will be no variability!}

%\item CMC: Coefficient of Multiple Correlation: Take for one class all curves for a person (8 curves) - compute CMC - get correlation coefficient per person - average over population. Low CMC for a given class means that the signals in this class have low similarity. 

%Compare different reliability scores. Are all consistent or are some of them contradictory?

%Which parameters can we use later and which ones are not suitable for averaging (because their  variation is too high)

%\subsection{Parameter Discriminativity} 

LDA was applied to the individual parameters and their combination, as well as to the higher-dimensional PCA-based representations. This analysis aimed at quantifying the discriminative power of the investigated representations and thereby evaluating their suitability for automated classification. Figure \ref{img:discriminativity} illustrates discriminativity scores obtained by LDA in terms of deviation from the random baseline (\textit{zero~rule}). In detail, results for different combinations of classes (rows) are illustrated: rows~1-4 provide results for the discrimination of normal gait vs. ankle, calcaneus, hip or knee (each class separately). Row~5 shows how well all 5 classes can be differentiated from each other. Row~6 illustrates how well normal gait can be differentiated from all types of gait disorders. Rows~7-12 show how all possible pairs of gait disorder classes can be differentiated from each other. 
%
%The analysis includes several tasks, covering all pairs of classes (e.g. N~vs.~C, N~vs.~\{C,~A,~H,~K\}, etc.) as well as a multi-class setting, i.e. N~vs.~C~vs.~A~vs.~K~vs.~H.
%
%Furthermore, the analysis comprises discriminativity scores for each parameter individually, for the combination of all parameters, as well as for the PCA representations and their combinations. 
Positive discriminativity scores are represented by a color scale from blue (corresponding to low values) to yellow (representing high values), whereas negative values are colored in gray. Positive values mean that the random baseline is exceeded and that the respective input parameter or input representation exhibits a certain discriminative power (the higher the value the better). Negative values indicate the absence of discriminative power, i.e. the random baseline is not reached. It has to be noted that, since the different class partitions represented by the rows of Figure~\ref{img:discriminativity} have different random baselines, the values across rows cannot be compared directly. Comparisons are solely valid along the rows. In general, however, columns including a larger number of high values indicate parameters or representations with a higher discriminative power. Similarly, rows with higher values represent tasks that are easier to solve than others.%, i.e. classes that are easier to distinguish. 

\begin{figure*}[ht!]
  \centering
	%\includegraphics[width=\textwidth]{images/discriminativity.pdf}
    \includegraphics[width=\textwidth]{images/discriminativity.png}
    \caption{Discriminativity scores obtained by LDA for different selections of classes (rows). The figure is divided into four blocks. Each column represents a different input parameter or higher-dimensional input representation. Best viewed in color.}
    \label{img:discriminativity}
\end{figure*}

The leftmost part of Figure~\ref{img:discriminativity} illustrates the discriminativity scores for the individual parameters. Several parameters achieve high scores for individual classes or combinations of classes, e.g. $F_{AP3}$, $F_{V3}$, $F_{VAVG}$, $F_{V1}$, $T_{V3}$, $T_{AP3}$, $GV$, $STEPV$, $DS$, $STRLEN$, $F_{V2}$, $STEPWD$, $CAD$, $BF$, and $STRIDET$. No parameter, however, performs well across all tasks. This indicates that individual parameters are quite limited in expressiveness. The second part ($ALL\_PARAMS$) of Figure~\ref{img:discriminativity} illustrates the results from the combination of all parameters. The combination yields much better discrimination across all rows of Figure~\ref{img:discriminativity}. This demonstrates that the individual parameters contain complementary information and attain synergies when they are combined. The third part of Figure~\ref{img:discriminativity} visualizes the results of the PCA-based representations of the five input signals $F_V$, $F_{AP}$, $F_{ML}$, $COP_{AP}$, and $COP_{ML}$. The three GRF components achieved higher scores compared to the COP signals. 
The rightmost part of Figure~\ref{img:discriminativity} shows the discriminativity scores for combined PCA representations, i.e all three GRF components combined ($PCA\_F_{ALL}$), both COP signals combined ($PCA\_COP_{AP,ML}$), and all five components combined ($PCA\_{ALL}$). In general, the combination of components improved the results, which indicates %shows 
that the individual GRF components are complementary to each other. The addition of the COP further improved the discriminative power. Thus, adding COP to a classification may contribute positively to the results. The %combined 
representations ($PCA\_{ALL}$ and $ALL\_PARAMS$) are %both 
combined able to contribute to all evaluated tasks (rows) of Figure~\ref{img:discriminativity}.

%The PCA-based representation of all GRF components, indicate higher discriminativity scores compared to the individual PCA-based representations, which also applies for the PCA-based representation of the combination of COP signals. The PCA-based representation of all five signals shows the highest discriminativity scores.   

The evaluated representations are more suitable for differentiating between the healthy control group and a functional gait disorder (rows 1-4) than between two functional gait disorders (rows 7-12). Regarding the task $N/GD$, solely a few parameters are able to exceed the random baseline. %The reason for this is
This is due to the fact that the combined set of all gait disorders contains much more samples than the class of healthy controls (i.e. 279 vs. 161 samples). This yields a random baseline around 87.1\% which is more difficult to exceed than random baselines in other tasks. 



%\todo[inline]{Djordje: for all datasets: A, B, C1, C2, C3: generate tables (Dev. from Random BL, Random BL, Total Acc.).}

%\begin{itemize}
%\item What do we want: high scores (higher is better).
%\item State what the random baseline is and say that everything above is good. Below is bad, i.e. the parameter does not explain anything in the data concerning our classes.
%\item What do columns with many high values represent? Very discriminative parameters
%\item What do rows with high values represent: Tasks that are easy
%\item Which parameters are strong, which are not and why?
%\item How is the behavior across all 5 classes?
%\item Which class can be distinguished best by the parameters
%\item Identify which parameters are most promising for a given Task
%\end{itemize}

%How large is the correlation between two parameters? Goal = dimension reduction (use Pearson correlation for this and CCA for the comparison of groups of parameters)

\subsection{Classification}
\label{subsec:classification}
%For the experiments in which PCA was utilized, different levels of explained variance were tested. For the final results, only the best suited approach , where 98\% of the variance was explained, was used.



The results of the classification experiments, which were performed on data from the test set, are summarized in Table \ref{tab:results}. The test set was not presented to the classifier during the training phase and the selection of its parameters. Results are provided for the two classification tasks ($N/C/A/K/H$ and $N/GD$) and for three different parameterizations. 
The results of the additional experiments with other classifiers such as the multi-layer perceptron (MLP) and the k-nearest neighbors algorithm (k-NN) were all outperformed by the SVM results, which confirms also the results of Janssen, Sch{\"o}llhorn et al. \cite{janssen2011diagnosing}. Therefore, and due to the limited space available, these results will not be discussed in detail.
%They provide a first baseline for the classification of functional gait disorders. 
%For task $N/GD$, the results of the RBF SVM for z-score and min-max normalized discrete parameters are below the random baseline (RB) and indicate that the respective model is not able to sufficiently explain the data. 

The first evaluated parameterization comprises of 52 GRF parameters (DPs and TDPs) that are extracted from all five GRF input signals. Due to the strong variation in the parameters' value ranges, a suitable normalization of the data is essential. We evaluated min-max normalization as well as z-standardization. The use of z-standardization resulted in a slightly higher deviation from the RB %classification accuracies 
for both tasks (except for the RBF SVM in task $N/C/A/K/H$) compared to min-max normalization. Furthermore, the RBF SVM failed to exceed the random baseline for both methods in the task $N/GD$.

The second parameterization was obtained by PCA of the raw GRF waveforms. PCAs obtained solely from the three force components clearly outperform the GRF parameters (DPs and TDPs). By adding the COP measurements the results were further improved for both tasks. Normalization of the PCA-based representations is crucial as performance otherwise drops significantly.

The third parameterization applied PCA on the z-standardized and min-max normalized DPs and TDPs. The dimensionality reduction resulted in a 28-dimensional vector which was also z-standardized prior to classification. In this case, results for both normalizations (last two rows of Table \ref{tab:results}) were improved for the task $N/GD$ compared to the representation with the original GRF parameters (first two rows of Table \ref{tab:results}).
%(rows 3-4). 
However, this is not the case for %the 
task $N/C/A/K/H$, where the deviation from the RB %accuracies 
slightly decreased. %slightly. 
%The use of z-standardization results in slightly higher accuracies for task $N/C/A/K/H$, whereas the min-max normalization allows higher accuracies for  
%This suggests that PCA removes redundant information and noise from the discrete parameters. Still, the performance level of PCA on the raw signals cannot be reached. 
%The PCA-based representation, which is obtained from the three GRF components, shows comparable results to the second experiment. Thus, PCA is capable of extracting important information from the whole waveforms. A slight improvement for both tasks  can be observed compared to the PCA on the discrete parameters.
%The PCA-based representation where PCA was performed on all five waveforms shows the best overall performances for both tasks. The highest classification accuracy for task $N/C/A/K/H$ is 53.22\% and is achieved with the RBF SVM. For task $N/GD$ the linear SVM provided the best performance with 90.33\%.
%The aim of the second experiment is to perform dimensionality reduction by applying PCA on the z-normalized discrete parameters. The resulting 29 dimensional vector is also z-normalized. The results indicate that the PCA removes redundant information and noise from the discrete parameters, thereby slightly improving the classification accuracies for both tasks (except for the linear SVM in task $N/C/A/K/H$). 

In summary, the best performance %classification accuracies 
(marked in bold in Table \ref{tab:results}) was achieved by applying PCA to all five GRF signals. The linear SVM achieved the highest deviation from the RB (22.5\%) for %the 
task $N/C/A/K/H$ as well as for %the 
task $N/GD$ (3.7\%).
%accuracy (54.31\%) for the task $N/C/A/K/H$ as well as for the task $N/GD$ (90.76\%).
Alternative classifiers which were also evaluated yielded a lower deviation from the RB: MLP~21.0\% and k-NN~13.4\% for %the 
task $N/C/A/K/H$ and MLP~2.6\% and k-NN~2.2\% for %the 
task $N/GD$. In terms of accuracy and deviation from the RB, the linear SVM performed better in all experiments. The RBF SVM has an advantage solely in terms of runtime.

%\new{The measured performances need to be interpreted with regards} to the random baseline which differs significantly for both tasks. While \new{in the case of the SVM} the random baseline \style{was} clearly exceeded for the first task (+22.5\%), the random baseline of the second task \style{was} only slightly exceeded (+3.7\new{\%}). The major reason for this is the strong class imbalance, which makes this task particularly difficult to solve. 
The main %major 
reason for the great difference in the performance  between the two tasks is the strong class imbalance in task $N/GD$, which makes this task particularly difficult to solve. 
One way of dealing with unbalanced datasets in SVMs is the use of different weights for different classes, thereby emphasizing the importance of the under-represented classes. Therefore, additional class-weighted experiments were performed. Results with different cost functions showed that no further performance increase can be achieved. The uniform cost function seems to work best on the data.

%Results after filtering the signals and normalizing to the foot length
\begin{table*}[ht!]
\centering
\caption{Classification results (\%) of two tasks - $N/C/A/K/H$ and $N/GD$ - and three different parameterization approaches. Note that the random baseline (RB) is stated next to the task name and that the values in the table represent the deviation from the random baseline (RB) and the corresponding absolute accuracy in brackets.}%Note that the random baseline (RB) is stated next to the task name and that the main content in the cell represents the deviation from the RB, whereas the value in the brackets is the absolute accuracy.}
\label{tab:results}
%\resizebox{1\textwidth}{!}{%
% \begin{tabular}{llc|cccc}
% \hline
% %\textbf{Parameterization} 						&	\textbf{Norm.} &	\textbf{Dim.} &	\multicolumn{2}{c}{$N/C/A/K/H$~(RB:~31.82\%)}  & \multicolumn{2}{c}{$N/GD$~(RB:~87.08\%)} \\ \hline

% \multicolumn{1}{l}{\multirow{2}{*}{\textbf{Parameterization}}} & \multicolumn{1}{l}{\multirow{2}{*}{\textbf{Norm.}}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Dim.}}} & \multicolumn{2}{c}{$N/C/A/K/H$~(RB:~31.8\%)}  & \multicolumn{2}{c}{$N/GD$~(RB:~87.1\%)} \\ \cline{4-7} 

% \multicolumn{3}{c|}{} 			& \multicolumn{1}{c}{\textbf{linear SVM}} & \multicolumn{1}{c}{\textbf{RBF SVM}}  & \multicolumn{1}{c}{\textbf{linear SVM}}   & \multicolumn{1}{c}{\textbf{RBF SVM}}     \\ \hline
% \rowcolor{gray!15}
% GRF Parameters (DPs and TDPs)	&	z-score	&	52 & 15.0\% (46.8\%) 	& 8.8\%	(40.6\%) &  2.4\% (89.5\%) & -0.8\% (86.3\%)\\
% GRF Parameters (DPs and TDPs)&	min-max	&	52 & 14.3\% (46.1\%)	&	9.5\% (41.3\%)  & 1.6\% (88.7\%)	& -3.8\% (83.3\%)\\
% \hline
% \rowcolor{gray!15}
% PCA on $F_{V}$, $F_{AP}$, $F_{ML}$ & z-score&	30	& 19.8\% (51.6\%)	&	15.4\% (47.2\%) & 2.4\% (89.5\%) & \textbf{2.0\% (89.1\%)}\\
% PCA on $F_{V}$, $F_{AP}$, $F_{ML}$, $COP_{AP}$, $COP_{ML}$ & z-score&	39 & \textbf{22.5\% (54.3\%)} &	\textbf{19.4\% (51.2\%)} & \textbf{3.7\% (90.8\%)} & 1.9\% (89.0\%)\\
% \hline
% \rowcolor{gray!15}
% PCA on z-standardized GRF parameters &	z-score&	28 & 13.8\% (45.6\%) &	8.8\% (40.6\%) & 2.6\% (89.7\%) & -0.6\% (86.5\%)\\
% PCA on min-max normalized GRF parameters &	z-score&	28 & 13.5\% (45.3\%) &	7.9\% (39.7\%) & 2.8\% (89.9\%) & 0.1\% (87.2\%)\\
% \hline
% \end{tabular}% <------ Don't forget this %
% %}
% \end{table*}
\begin{tabular}{llc|cccc}
\hline
%\textbf{Parameterization} 						&	\textbf{Norm.} &	\textbf{Dim.} &	\multicolumn{2}{c}{$N/C/A/K/H$~(RB:~31.82\%)}  & \multicolumn{2}{c}{$N/GD$~(RB:~87.08\%)} \\ \hline

\multicolumn{1}{l}{\multirow{2}{*}{\textbf{Parameterization}}} & \multicolumn{1}{l}{\multirow{2}{*}{\textbf{Norm.}}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Dim.}}} & \multicolumn{2}{c}{$N/C/A/K/H$~(RB:~31.8\%)}  & \multicolumn{2}{c}{$N/GD$~(RB:~87.1\%)} \\ \cline{4-7} 

\multicolumn{3}{c|}{} 			& \multicolumn{1}{c}{\textbf{linear SVM}} & \multicolumn{1}{c}{\textbf{RBF SVM}}  & \multicolumn{1}{c}{\textbf{linear SVM}}   & \multicolumn{1}{c}{\textbf{RBF SVM}}     \\ \hline
\rowcolor{gray!15}
GRF Parameters (DPs and TDPs)	&	z-score	&	52 & 15.0 (46.8) 	& 8.8	(40.6) &  2.4 (89.5) & -0.8 (86.3)\\
GRF Parameters (DPs and TDPs)&	min-max	&	52 & 14.3 (46.1)	&	9.5 (41.3)  & 1.6 (88.7)	& -3.8 (83.3)\\
\hline
\rowcolor{gray!15}
PCA on $F_{V}$, $F_{AP}$, $F_{ML}$ & z-score&	30	& 19.8 (51.6)	&	15.4 (47.2) & 2.4 (89.5) & \textbf{2.0 (89.1)}\\
PCA on $F_{V}$, $F_{AP}$, $F_{ML}$, $COP_{AP}$, $COP_{ML}$ & z-score&	39 & \textbf{22.5 (54.3)} &	\textbf{19.4 (51.2)} & \textbf{3.7 (90.8)} & 1.9 (89.0)\\
\hline
\rowcolor{gray!15}
PCA on z-standardized GRF parameters &	z-score&	28 & 13.8 (45.6) &	8.8 (40.6) & 2.6 (89.7) & -0.6 (86.5)\\
PCA on min-max normalized GRF parameters &	z-score&	28 & 13.5 (45.3) &	7.9 (39.7) & 2.8 (89.9) & 0.1 (87.2)\\
\hline
\end{tabular}% <------ Don't forget this %
%}
\end{table*}


%\begin{itemize}
%\item Performance of discrete parameters (all)
%\item Performance of discrete parameters (most promising subset from our discriminativity analysis)
%\item Performance of PCA at different levels of explained variance (e.g. 90\%, 95\% and 98\%). Discuss results and say how many  PCs the different levels of explained variance correspond to. Show a plot of explained variance for each PC (simply ``plot(explained)" - this could be interesting)
%\item PCA on discrete parameters (motivation: denoising and dimensionality reduction)
%\item Combine PCA with discrete Parameters? Do we want to show that already or keep it for a follow up paper?
%\item Confusion Matrix: show confusion matrix (if space available). If not: just discuss where most confusions occur and hypothesize why.
%\item For each experiment provide accuracy for linear SVM and rbf SVM. Mention random baseline also
%\item If space: show examples of correctly and falsely classified patterns
%\end{itemize}

\subsection{Discussion and further aspects} 
%This study aimed at classifying a total of five patient classes with different orthopedic conditions. In contrast to previous research \textbf{(add Refs here)} this study utilized rather broad inclusion criteria for each class. 
We presented a study on the classification of different functional gait disorders, stemming from a wide range of possible impairments, into categories that represent the main affected body region. The motivation for selecting these broad categories is that identifying the region of impairment is essential for clinical practice and may allow to pinpoint impairments already at an early stage. In addition, it could indicate secondary impairments which may easily be overlooked by the physician during clinical examination. The present study represents a first performance baseline for the classification of gait disorders. Results are particularly promising for %the 
task $N/GD$. However, an absolute classification accuracy of 91\% still lies below an acceptable threshold for clinical practice. For the classification of individual disorder categories, the results indicate that further improvements are necessary. To date, the proposed approach could, however, already serve as a support for clinicians indicating the presence of (additional) arthropathies or diseases. 
%\todo[inline]{Ich weiss nicht ob das hier reinpasst! Was? Das oben oder das unten?}
In order to reduce the classification complexity, while still providing support for clinicians, similar classes could be merged, i.e. the hip and knee classes into a thigh class and the ankle and calcaneus classes into a shank class. The results of this additional experiment showed a deviation from the RB of 26.8\% (using a linear SVM, RB:~51\%, absolute accuracy:~77.8\%). Compared to the distinction of all five classes ($N/C/A/K/H$), this is a clear increase in accuracy and deviation from the RB.

Different influencing factors, i.e. the imbalance of the class priors, the variability in the number of sessions per person and gender-specific aspects may introduce a bias into the aforementioned analyses. To investigate the effect of these factors on classification performance, we performed additional experiments. To this end, we used the best configuration found so far as a baseline, i.e. PCA on all five signals with a linear SVM (4th parametrization in Table \ref{tab:results}) and applied it to different balanced subsets of our dataset. The results are presented in Table~\ref{tab:results2} and are discussed in the following.  

\begin{table}[ht!]
\centering
\caption{Results (\%) of analyses assessing the influence of several factors on the results of the two tasks - $N/C/A/K/H$ and $N/GD$. The experiments are performed with a PCA on all five signals in combination with a linear SVM. Note that the values represent the deviation from the random baseline (RB) and the corresponding absolute accuracy in brackets.}%Note that the main content in the cell represents the deviation from the random baseline (RB), and the value in the brackets the absolute accuracy.}}
\label{tab:results2}
%\resizebox{1\textwidth}{!}{%
\begin{tabular}{l|cc}
\hline
\textbf{Partitions of the dataset}                                           & $N/C/A/K/H$ & $N/GD$ \\
\hline
\rowcolor{gray!15}
Session are balanced                       &     23.7 (60.2)      &  20.6 (84.1)   \\
Persons are balanced                       &      28.3 (59.5)     &      5.3 (84.7)\\
\rowcolor{gray!15}
Persons \& sessions are balanced &     39.2 (59.2)      &    35.4 (85.4) \\
Male population                                                        &     20.9 (51.3)     &   0.6 (91.4)  \\
\hline
\end{tabular}% <------ Don't forget this %
%}
\end{table}


For the experiments in Section \ref{subsec:classification} we decided to use all available sessions of patients recorded in the course of their rehabilitation to account for different progression stages of impairments. This, however, may introduce a bias in the experiments as  more trials exist for some patients than for others. To evaluate to which extent the varying number of recorded sessions per patient influences the overall result, we balanced the dataset by selecting only one random session per person. Interestingly, the deviation from the RB improved for task~$N/C/A/K/H$ to 23.7\% (+1.2\%) and for task~$N/GD$ to 20.6\% (+16.9\%), as presented in the first row of Table~\ref{tab:results2}. These results show that intra-patient variability needs to be taken into account and requires additional modeling in a classification approach.
%Interestingly, this led to an increase of the deviation from the RB for task~$N/GD$ to 20.6\% (linear SVM, RB:~63.5\%, absolute accuracy:~84.1\%) and for task~$N/C/A/K/H$ to 23.7\% (linear SVM, RB:~36.5\%, absolute accuracy:~60.2\%).

Another factor causing an imbalance in the data are the different class cardinalities, i.e. different numbers of persons per class.
%Even though a large number of measurements is used to train the classifiers, the present imbalance in the data regarding the class cardinalities challenges automated classification (especially for the task~$N/GD$). 
%Results may be further improved by balancing the dataset with additional samples, which is subject to our ongoing work. 
In order to investigate the influence of this imbalance we performed an experiment for both tasks with a dataset containing the same number of participants per class (but keeping all sessions in the dataset).  
For task~$N/C/A/K/H$ the balanced dataset is composed of data from 62 persons from each class (overall 310 persons, 7616 trials).
%62 persons per class (A:259 sessions C:234 sessions H:168 sessions K:229 sessions
For task~$N/GD$ the balanced dataset contained data from 160 healthy controls and 160 persons with a deficit (40 from each GD class,  overall 320 persons and 6096 trials).
%160 normal, 40 persons per class (A: 168 sessions, C: 164 sessions, H: 119 sessions, K: 151 sessions)
The deviation from the RB improved for task~$N/C/A/K/H$ to 28.3\% (+5.8\%) and for task~$N/GD$ to 5.3\% (+1.6\%), as shown in the second row of Table~\ref{tab:results2}. Although the results show that balancing the number of patients among classes is beneficial, the results of task~$N/GD$ reveal the still existing imbalance in the dataset (due to the fact that healthy controls have only one session and patients up to several sessions).   

%These results show that balancing the number of patients among classes is beneficial, compared to using unbalanced classes. }

The next question deals with the effect of balancing the number of patients and the number of sessions at the same time. We performed experiments with a completely balanced version of our dataset for each task, containing only one session per person and equal numbers of persons per class. For task~$N/C/A/K/H$ the balanced dataset is composed of data from 62 persons from each class (overall 310 persons, 2480 trials). For task~$N/GD$ the balanced dataset contained data from 160 healthy controls and 160 persons with a deficit (40 from each GD class,  overall 320 persons and 2560 trials). The results of our experiments showed clear performance improvements of +16.7\% in the deviation from the RB compared to the baseline for task $N/C/A/K/H$ and +31\% compared to the baseline for task $N/GD$ (see the third row in Table~\ref{tab:results2}). 
%\new{In order to investigate the imbalance of class cardinalities we performed experiments with a completely balanced version of our dataset for each task, containing only one session per person and equal numbers of persons per class. For task~$N/GD$ the balanced dataset (320 persons, 2560 trials) contained data from 160 healthy controls and 160 persons with a deficit (40 from each GD class). For task~$N/C/A/K/H$ the balanced dataset is composed of data from 62 persons from each class (overall 310 persons, 2480 trials). The results of our experiments showed clear performance improvements. The deviation from the RB for task~$N/GD$ increased to 35.4\% (linear SVM, RB:~50\%, absolute accuracy:~85.4\%) and for task~$N/C/A/K/H$ to 39.2\% (linear SVM, RB:~20\%, absolute accuracy:~59.2\%). Future work of our group will focus on establishing a big, open-source, and balanced data set to foster further developments in this area.} 

Other biases in the data may be introduced by variations in gender, walking velocity, leg length and other parameters \cite{pierrynowski_enhancing_2001} leading to a variability of GRF parameterizations in the individual disorder classes. Additional normalization of the input data may be necessary to reduce intra-class variation to improve classification accuracy. Several studies have shown that in particular gender causes strong variability in gait signals~\cite{eskofier2012pattern,chiu2007effect}. To assess the influence of gender on our results, an experiment was performed on a reduced dataset containing only data from male participants (note that the number of female participants in our dataset is not sufficient to perform separate experiments). Surprisingly, the results did not improve (see the last row in Table~\ref{tab:results2}). This indicates that for our data, gender has rather little influence on the results, which, however, does not imply that the influence of gender can be neglected a priori. A detailed study on the influence of gender is subject to future investigation.
%The deviation from the RB for task~$N/GD$ is 0.6\% (RBF SVM, RB:~90.8\%, absolute accuracy:~91.4\%) and for task~$N/C/A/K/H$ the deviation is 20.9\% (linear SVM, RB:~30.4\%, absolute accuracy:~51.3\%).

%\todo[inline]{find the right place for this}


% A reason may be the unequal assignment of female participants in the different classes. 
%This indicates, that the combined analysis of both genders does not affect the classification accuracy. However, it is noteworthy, that we cannot conclude from these results, that gender does not have a general impact on the data.
%compared to the influence of the different functional deficits.}
%\todo[inline]{Sollten wir mit Matthias besprchen (BRian)}



%Information solely based on GRF may be not enough to clearly distinguish these classes. Here additional information derived from three-dimensional gait analysis may perhaps be necessary. 
%However, future research may build upon our results and may follow different strategies to reach our proposed aim. 

%\subsection{Comparison with previous studies}
%
%\todo[inline]{QUESTION: will this be part of paper? Is this rather a discussion or a comparison with additional experiments, e.g. apply other method on our data}

%Are we consistent with previous studies? What is different? Are there novel insights?


==> Automatic Classification of Functional Gait Disorders/06_conclusion.tex <==
\IEEEPARstart{T}{he} present study aimed at classifying patients with different orthopedic gait impairments at the hip, knee, ankle, and calcaneus from healthy controls using GRF measurements. For this purpose a dataset of 9,496 gait measurements from clinical practice was utilized. In a first step we investigated the suitability of state-of-the-art GRF parameterizations and analyzed their statistical properties and discriminative power among the classes. %The results suggest
Based on these results, the use of entire GRF waveform parameterizations as input (such as PCA), rather than relying on GRF parameters (DPs and TDPs) seems advisable. Furthermore, the use of GRF force components paired with the respective COP measurements yielded the best results. Our experiments further showed that balancing the dataset significantly improves results (e.g. increasing the deviation from the random baseline by +16.7\% for the classification into healthy controls and all four GD classes and by +31\% for distinguishing between healthy controls and patients).
%The distinction between healthy controls and patients reached an accuracy of approximately 91\%. \style{By contrast, the comparison of the healthy controls with all four GD classes reached a classification accuracy of 54\%.} %, while an accuracy of 54\% was achieved for classification between healthy gait and all four GD classes.
 
The presented study shows that results heavily depend on the employed GRF representation. Future work will investigate and evaluate adaptively learned signal representations \cite{zhang2013pathological,hannink2017sensor} to obtain more discriminative and expressive parameterizations of GRF measurements. Furthermore, we will focus on establishing a large, open-source, and balanced data set to foster further developments in this area. Our results thereby provide a first performance baseline for the classification of functional gait disorders and can serve as a reference for future improvements.

